Counterfactual Zero-Shot and Open-Set Visual Recognition

We present a novel counterfactual framework for both Zero-Shot Learning (ZSL) and Open-Set Recognition (OSR), whose common challenge is generalizing to the unseen-classes by only training on the seen-classes. Our idea stems from the observation that the generated samples for unseen-classes are often out of the true distribution, which causes severe recognition rate imbalance between the seen-class (high) and unseen-class (low). We show that the key reason is that the generation is not Counterfactual Faithful, and thus we propose a faithful one, whose generation is from the sample-specific counterfactual question: What would the sample look like, if we set its class attribute to a certain class, while keeping its sample attribute unchanged? Thanks to the faithfulness, we can apply the Consistency Rule to perform unseen/seen binary classification, by asking: Would its counterfactual still look like itself? If ``yes'', the sample is from a certain class, and ``no'' otherwise. Through extensive experiments on ZSL and OSR, we demonstrate that our framework effectively mitigates the seen/unseen imbalance and hence significantly improves the overall performance. Note that this framework is orthogonal to existing methods, thus, it can serve as a new baseline to evaluate how ZSL/OSR models generalize. Codes are available at https://github.com/yue-zhongqi/gcm-cf.

==> figures/figure6.tex <==
\begin{figure}[h!]

    \centering
    \captionsetup{font=footnotesize,labelfont=footnotesize,skip=5pt}

    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=0.98\textwidth]{figures/exp_fig1a.pdf}
        \caption{CUB~\cite{WelinderEtal2010}}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=0.98\textwidth]{figures/exp_fig1a.pdf}
        \caption{AWA2~\cite{xian2018zero}}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=0.98\textwidth]{figures/exp_fig1a.pdf}
        \caption{SUN~\cite{xiao2010sun}}
    \end{subfigure}%
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=0.98\textwidth]{figures/exp_fig1a.pdf}
        \caption{aPY~\cite{farhadi2009describing}}
    \end{subfigure}
    
    \caption{The Seen-Unseen accuracy Curve (SUC) together with the Area Under SUC (AUSUC) on the four datasets. The cross denotes the ZSL Accuracy when calibration factor $\omega$=0.}
    \label{fig:6}
\end{figure}

==> tables/closed_set.tex <==
\begin{table}[t]
\centering
\captionsetup{font=footnotesize,labelfont=footnotesize,skip=5pt}
\scalebox{0.73}{
\begin{tabular}{p{2.5cm} p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}}
%{cl|cccccc|cccccc}
\hline\hline
\large{Method} & MNIST & SVHN & CIFAR10 & C+10 & C+50 \\
\hline
Plain CNN & 0.995 & 0.965 & 0.917 & 0.941 & 0.940 \\
CGDL~\cite{sun2020conditional} & 0.996 & 0.962 & 0.913 & 0.934 & 0.935 \\
%\textbf{GCM-CF} (Ours) & 0.996 & 0.963 & 0.918 & 0.935 & 0.933 \\
\hline \hline
\end{tabular}}
\caption{Comparison of the Closed-Set accuracy in OSR.}
\label{tab:4}
\vspace{-0.3cm}
\end{table}

==> tables/osr/close_set_5.tex <==
\begin{table}[t]
\centering
\captionsetup{font=footnotesize,labelfont=footnotesize,skip=5pt}
\scalebox{0.73}{
\begin{tabular}{p{2.5cm} p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}}
%{cl|cccccc|cccccc}
\hline\hline
\multicolumn{1}{c}{Split} & \multicolumn{5}{c}{1} \\
\hline
\multicolumn{1}{c}{Method} & MNIST & SVHN & CIFAR10 & C+10 & C+50 \\
\hline
Plain CNN & 0.995 & 0.965 & 0.917 & 0.941 & 0.940 \\
CGDL~\cite{sun2020conditional} & 0.996 & 0.963 & 0.902 & 0.929 & 0.934 \\
\hline \hline

\multicolumn{1}{c}{Split} & \multicolumn{5}{c}{2} \\
\hline
\multicolumn{1}{c}{Method} & MNIST & SVHN & CIFAR10 & C+10 & C+50 \\
\hline
Plain CNN & 0.995 & 0.965 & 0.917 & 0.941 & 0.940 \\
CGDL~\cite{sun2020conditional} & 0.995 & 0.966 & 0.940 & 0.933 & 0.932 \\
\hline \hline

\multicolumn{1}{c}{Split} & \multicolumn{5}{c}{3} \\
\hline
\multicolumn{1}{c}{Method} & MNIST & SVHN & CIFAR10 & C+10 & C+50 \\
\hline
Plain CNN & 0.995 & 0.965 & 0.917 & 0.941 & 0.940 \\
CGDL~\cite{sun2020conditional} & 0.996 & 0.963 & 0.934 & 0.939 & 0.940 \\
\hline \hline

\multicolumn{1}{c}{Split} & \multicolumn{5}{c}{4} \\
\hline
\multicolumn{1}{c}{Method} & MNIST & SVHN & CIFAR10 & C+10 & C+50 \\
\hline
Plain CNN & 0.995 & 0.965 & 0.917 & 0.941 & 0.940 \\
CGDL~\cite{sun2020conditional} & 0.997 & 0.958 & 0.923 & 0.934 & 0.931 \\
\hline \hline

\multicolumn{1}{c}{Split} & \multicolumn{5}{c}{5} \\
\hline
\multicolumn{1}{c}{Method} & MNIST & SVHN & CIFAR10 & C+10 & C+50 \\
\hline
Plain CNN & 0.995 & 0.965 & 0.917 & 0.941 & 0.940 \\
CGDL~\cite{sun2020conditional} & 0.996 & 0.959 & 0.865 & 0.935 & 0.939 \\
\hline \hline
\end{tabular}}
\caption{Comparison of the Closed-Set accuracy in OSR.}
\label{tab:4}
\vspace{-0.3cm}
\end{table}
